Multi-Behavior Recommender Systems: A Survey

Traditional recommender systems primarily rely on a single type of user-item interaction, such as item purchases or ratings, to predict user preferences. However, in real-world scenarios, users engage in a variety of behaviors, such as clicking on items or adding them to carts, offering richer insights into their interests. Multi-behavior recommender systems leverage these diverse interactions to enhance recommendation quality, and research on this topic has grown rapidly in recent years. This survey provides a timely review of multi-behavior recommender systems, focusing on three key steps: (1) Data Modeling: representing multi-behaviors at the input level, (2) Encoding: transforming these inputs into vector representations (i.e., embeddings), and (3) Training: optimizing machine-learning models. We systematically categorize existing multi-behavior recommender systems based on the commonalities and differences in their approaches across the above steps. Additionally, we discuss promising future directions for advancing multi-behavior recommender systems.

==> 030procedure.tex <==
\subsection{Task Description}
Multi-behavior recommendation aims to predict interactions for a target behavior (e.g., purchases) based on the interactions observed in auxiliary behaviors (e.g., clicks, adds-to-cart, collects). This task leverages the interplay between multiple types of user behavior to enhance the accuracy and reliability of recommendations. By integrating signals from diverse behaviors, models can better capture user preferences, even when data for the target behavior is sparse or noisy.

\subsubsection{Key Steps} Multi-behavior recommendation generally involves three key steps. First, it focuses on modeling the various relationships (e.g., clicks, adds-to-cart, collects, dislikes) between user behaviors to predict a target behavior (e.g., purchases). These relationships are typically represented through diverse data structures that capture the interactions and dependencies between different behaviors. Second, the encoded data is transformed into a meaningful representation that can be used for recommendation. This encoding can be achieved through a variety of techniques, including Matrix Factorization (MF), Graph Neural Networks (GNNs), Recurrent Neural Networks (RNNs), and Transformer-based models. Each encoding method has its strengths and is chosen based on the characteristics of the data and the task at hand. Finally, the training objectives are defined. These objectives are broadly categorized into main objectives focused on optimizing recommendation performance and auxiliary objectives that leverage additional features to enhance the model's learning. Auxiliary objectives may include self-supervised tasks, contrastive learning, or generative learning to improve model robustness and the quality of learned representations. 

In this survey, we provide a comprehensive examination of existing approaches for each of these three steps in multi-behavior recommendation. We categorize the methods systematically and analyze the different strategies employed to achieve effective recommendations. Figure~\ref{fig:framework} illustrates the overall procedure of multi-behavior recommendation, while Table~\ref{tab:datasets} summarizes the key characteristics of existing works in this field.

\begin{figure}
\includegraphics[width=\textwidth]{FIG/Framework_v0.2.pdf}
\caption{Procedure of multi-behavior recommendation.} \label{fig:framework}
\end{figure}


==> TABLES/old_summary.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}
    \small
    \centering
    \setlength{\tabcolsep}{8pt}
    \caption{Summary of multi-behavior recommender systems.}
    %\rowcolors{2}{gray!20}{white}
    \label{tab:summary}
    \begin{tabular}{l|c c c c|c c c|c c c}
        \hline
        \toprule
        & \multicolumn{4}{c|}{\textbf{Modeling}} 
        & \multicolumn{3}{c|}{\textbf{Encoding}} 
        & \multicolumn{3}{c}{\textbf{Aux. Objective}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        \textbf{Model} 
        & \rotatebox{90}{\shortstack{\textbf{View-Specific} \\ \textbf{Graphs}}} 
        & \rotatebox{90}{\shortstack{\textbf{View-Unified} \\ \textbf{Graph}}} 
        & \rotatebox{90}{\shortstack{\textbf{View-Unified} \\ \textbf{Sequences}}} 
        & \rotatebox{90}{\textbf{Others}} 
        & \rotatebox{90}{\textbf{Parallel}} 
        & \rotatebox{90}{\textbf{Sequential}} 
        & \rotatebox{90}{\textbf{Others}} 
        & \rotatebox{90}{\textbf{Aux. Ranking}} 
        & \rotatebox{90}{\textbf{Contrastive}} 
        & \rotatebox{90}{\textbf{Generative}} \\
        \midrule
        \rowcolor{gray!20} CMF~\cite{singh2008relational} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        MR-BPR~\cite{Krohn-Grimberghe2012multi} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MC-BPR~\cite{loni2016bayesian} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        BPRH~\cite{qiu2018bprh} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} VALS~\cite{ding2018improving} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes}\\
        BINN~\cite{li2018learning} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} NMTR~\cite{gao2019neural} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        DIPN~\cite{guo2019buying} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MRMN~\cite{zhou2019collaborative} &\textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        MATN~\cite{xia2020multiplex} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MBGCN~\cite{jin2020multi} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        EHCF~\cite{chen2020efficient} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MGNN~\cite{zhang2020multiplex} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes}\\
        GMNR~\cite{xia2021multi} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MB-GMN~\cite{xia2021graph} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        HMG-CR~\cite{yang2021hyper} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} GHCF~\cite{chen2021graph} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        KHGT~\cite{xia2021knowledge} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} S-MBRec~\cite{gu2022self} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        CML~\cite{wei2021contrastive} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MB-STR~\cite{yuan2022multi} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck}\\
        MBHT~\cite{yang2022multi} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} \\
        \rowcolor{gray!20} MMCLR~\cite{wu2022multi} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        CKML~\cite{meng2023coarse} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} CRGCN~\cite{meng2023coarse} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        MB-CGCN~\cite{cheng2023multi}  & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} PKEF~\cite{meng2023parallel} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        HPMR~\cite{meng2023hierarchical} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} CHCF~\cite{luo2023criterion} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        %MbSRS~\cite{zhao2023mbsrs} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        MB-HGCN~\cite{yan2023mbhgcn} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} PBAT~\cite{su2023personalized} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        KMVLR~\cite{xuan2023knowledge} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MBA~\cite{xin2023improving} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} &\textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\ 
        MBSSL~\cite{xu2023multi} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} BCIPM~\cite{yan2024behavior} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        END4Rec~\cite{han2024efficient} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} MBGen~\cite{liu2024multi} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} \\
        MULE~\cite{lee2024mule} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} DA-GCN~\cite{zhu2024multi} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        HMAR~\cite{elsayed2024hmar} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \rowcolor{gray!20} PO-GCN~\cite{zhang2024multi} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} & \textcolor{green}{\faCheck} & \textcolor{red}{\faTimes} & \textcolor{red}{\faTimes} \\
        \bottomrule
        \hline
    \end{tabular}
\end{table}
